Zero-shot Sim2Real Adaptation Across Environments

Simulation based learning often provides a cost-efficient recourse to reinforcement learning applications in robotics. However, simulators are generally incapable of accurately replicating real-world dynamics, and thus bridging the sim2real gap is an important problem in simulation based learning. Current solutions to bridge the sim2real gap involve hybrid simulators that are augmented with neural residual models. Unfortunately, they require a separate residual model for each individual environment configuration (i.e., a fixed setting of environment variables such as mass, friction etc.), and thus are not transferable to new environments quickly. To address this issue, we propose a Reverse Action Transformation (RAT) policy which learns to imitate simulated policies in the real-world. Once learnt from a single environment, RAT can then be deployed on top of a Universal Policy Network to achieve zero-shot adaptation to new environments. We empirically evaluate our approach in a set of continuous control tasks and observe its advantage as a few-shot and zero-shot learner over competing baselines.

==> readme.tex <==
\subsection*{Prerequisites}

Python 3.7

(From \url{https://github.com/VincentYu68/policy_transfer})

\begin{itemize}
\item OpenAI Baselines (https://github.com/openai/baselines) 
\item MuJoCo Simulator (https://github.com/openai/mujoco-py)
\item OpenAI Gym (https://github.com/openai/gym)
\end{itemize}
Instructions for installing OpenAI Baselines: https://github.com/openai/baselines. 

\subsection*{Installation}

Run the following command from the project directory:

\begin{verbatim}
cd reverse_action_transform
pip install -e .
source setup.sh
\end{verbatim}		

For parameter descriptions for the commands please refer to the Section \emph{Parameter Descriptions for Commands}. 

\textbf{All trained agents can be found in \emph{trained\_agents} directory. Code root directory is \emph{reverse\_action\_transform}}. Prior to running following scripts, copy the content in \emph{trained\_agents/trained\_upns} to the code root.

\subsection{\label{sec:upn_train} Trained Universal Policy Networks (UPNs)}

The set of UPNs trained in the simulator for $2\times10^8$ steps and fine-tuned for $5 \times 10^6$ steps at the ground-truth parameter value is given in \emph{./data\_mujoco\_205m\_pretrained\_10kbatch\_160722/} directory. For Walker2D task, use the \emph{./data\_mujoco\_206m\_pretrained\_10kbatch\_20722/} since we used the $6\times10^6$ steps UPN version.

\subsection{\label{sec:eval-rat} Hyperparameter Tuning with Bayesian Optimisation (BO)}

To optimise hyperparameters \emph{clip}, \emph{entcoeff}, \emph{stepsize}, \emph{lambda} and \emph{gamma} with Bayesian Optimisation (BO) for \emph{Robust Initial RAT policy} learning, first set the \emph{RAT} training directives in \emph{policy\_transfer/reality\_mod/rat/rat.py}.

\begin{verbatim}
DR_latent_resample = Trie
DR_latent_params = [0, 1] # friction, mass
DR_latent_range = [[0, 0], [1.0, 3.0]] #[low, high]
\end{verbatim}

To control simulation state resetting to the real-world at each timestep ($reset$ option in Algo. 1 in the paper), comment out lines 84 and 85 in \emph{policy\_transfer/reality\_mod/rat/ppo\_rat.py} script to disable resetting.

\begin{verbatim}
env_sim.env.set_state_vector(env_real.env.state_vector())
ob_sim = ob
\end{verbatim}

To change the number of hidden layers in \emph{RAT} policy network, change the \emph{num\_hid\_layers} parameter in function \emph{policy\_fn2} in \emph{policy\_transfer/reality\_mod/rat/rat.py} (lines 314), \emph{policy\_transfer/reality\_mod/rat/eval\_rat.py} (line 350) and \emph{policy\_transfer/reality\_mod/rat/mod\_rat\_mt.py} (line 224). We have used $5$ (Ant, Swimmer, Walker) and $10$ (Half-Cheetah, Hopper, Humanoid) layer sizes of $128$ neurons for task environments.

\

Then run the following scripts for respective tasks with passing one command line argument for the file path containing the ground-truth parameter values used for \emph{--real\_latent} and \emph{--sim\_latent}. Ground truth parameter values are given in \emph{results/gt\_seed\_0.json}.

\begin{itemize}
\item Ant: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_ant\_5d.sh}
\item Half-Cheetah: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_cheetah\_5d.sh}
\item Hopper: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_hopper\_5d.sh}
\item Humanoid: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_humanoid\_5d.sh}
\item Swimmer: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_swimmer\_5d.sh}
\item Walker2D: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_walker2d\_5d\_206m.sh}
\end{itemize}


At the end of a hyperparameter tuning run, the program will print the directory in which the results are saved. In the folder, results of BO evaluations will be saved in a file \emph{results-*.csv}. All trained \emph{RAT} agents for BO trials with different hyperparameter value will be saved in folders \emph{train\_*\_[id]} where \emph{[id]} corresponds to the BO trial iteration in the results file. We used the best RL agent from \emph{Robust RAT Initial Policy} learning for zero-shot adaptation. \textbf{These tuned agents are available in \emph{trained\_agents/rat\_priors} directory.}

\subsection{\label{sec:eval-rat} Evaluating a Trained \emph{RAT} Policy}

This command will evaluate a \emph{RAT} policy using a given number of trials on the real-world. Run the following scripts for six environments with passing two command line arguments: 1) the path to the \emph{RAT} policy, and 2) file path containing the ground-truth parameter values used for \emph{--real\_latent} and \emph{--sim\_latent},

\begin{itemize}
\item Ant: \emph{./scripts/no\_grounding2/eval\_rat\_ant\_5d.sh}
\item Half-Cheetah: \emph{./scripts/no\_grounding2/eval\_rat\_cheetah\_5d.sh}
\item Hopper: \emph{./scripts/no\_grounding2/eval\_rat\_hopper\_5d.sh}
\item Humanoid: \emph{./scripts/no\_grounding2/eval\_rat\_humanoid\_5d.sh}
\item Swimmer: \emph{./scripts/no\_grounding2/eval\_rat\_swimmer\_5d.sh}
\item Walker2D: \emph{./scripts/no\_grounding3/eval\_rat\_walker\_5d.sh}
\end{itemize}

% Data to provide
% *) data mujoco 205m pretrained 10kbatch 160722 (x)
% *) data mujoco 206m pretrained 10kbatch 160722
% *) data mujoco 207m pretrained 10kbatch 160722
% *) drift envs
% *) robust-prior-hyperparam-optimal-agent
% *) RAT 20k adapted optimal agent
% *) UPN transfer agents trained for 20k


\subsection{\label{sec:zero-shot} Zero-shot Evaluation of \emph{RAT} Policy to Adjacent Environments}

To evaluate zero-shot transfer on adjacent environments (i.e., drift environments), we generate $100$ such uniformly sampled environments $\pm5\%$ from the ground truth. For each of the environments, run the following commands or use the provided environment samples in \textbf{ \emph{trained\_agents/drift\_envs}.}

\begin{itemize}
\item Ant: \emph{./scripts/drift\_search/no\_ground/drift\_search\_ant\_5d.sh}
\item Half-Cheetah: \emph{./scripts/drift\_search/no\_ground/drift\_search\_cheetah\_5d.sh}
\item Hopper: \emph{./scripts/drift\_search/no\_ground/ drift\_search\_hopper\_5d.sh}
\item Humanoid: \emph{./scripts/drift\_search/no\_ground/ drift\_search\_humanoid\_5d.sh}
\item Swimmer: \emph{./scripts/drift\_search/no\_ground/ drift\_search\_swimmer\_5d.sh}
\item Walker2D: \emph{./scripts/drift\_search/no\_ground/ drift\_search\_walker\_5d.sh}
\end{itemize}


Then run the following scripts for six environments with passing two command line arguments: 1) the path to the trained \emph{RAT} initial policy, and 2) the path to respective adjacent environments file generated in the earlier step. Within the context of this script, \emph{--sim\_latent} refers to the "adjacent environments file" and not to the ground truth parameters, as used in rest of the scripts.

\begin{itemize}
\item Ant: \emph{./scripts/mod\_env/real\_world\_upn205m/mod\_env\_mt\_ant\_5d.sh}
\item Half-Cheetah: \emph{./scripts/mod\_env/real\_world\_upn205m/mod\_env\_mt\_cheetah\_5d.sh}
\item Hopper: \emph{./scripts/mod\_env/real\_world\_upn205m/mod\_env\_mt\_hopper\_5d.sh}
\item Humanoid: \emph{./scripts/mod\_env/real\_world\_upn205m/mod\_env\_mt\_humanoid\_5d.sh}
\item Swimmer: \emph{./scripts/mod\_env/real\_world\_upn205m/mod\_env\_mt\_swimmer\_5d.sh}
\item Walker2D: \emph{./scripts/mod\_env/real\_world\_upn206m/mod\_env\_mt\_walker\_5d.sh}
\end{itemize}


\subsection{\label{sec:mujoco_ids} MuJoCo Task IDs}

\subsubsection{Ant}
	\begin{itemize}
		\item Env ID: AntPT-v2	
		\item Simulation parameter IDs: 0, 1, 2, 8, 16
	\end{itemize}


\subsubsection{Half-Cheetah}
	\begin{itemize}
		\item Env ID: HalfCheetahPT-v2	
		\item Simulation parameter IDs: 0, 1, 4, 7, 8
	\end{itemize}
	
\subsubsection{Hopper}
	\begin{itemize}
		\item Env ID: HopperPT-v2
		\item Simulation parameter IDs: 0, 1, 2, 3, 10			
	\end{itemize}

\subsubsection{Humanoid}
	\begin{itemize}
		\item Env ID: HumanoidPT-v2	
		\item Simulation parameter IDs: 0, 1, 6, 9, 14
	\end{itemize}

\subsubsection{Swimmer}
	\begin{itemize}
		\item Env ID: SwimmerPT-v2	
		\item Simulation parameter IDs: 0, 1, 2, 3, 6
	\end{itemize}

\subsubsection{Walker2D}
	\begin{itemize}
		\item Env ID: Walker2dPT-v2	
		\item Simulation parameter IDs: 0, 1, 2, 7, 8
	\end{itemize}
\pagebreak\clearpage{}


\subsection{\label{sec:param-desc} Parameter Descriptions for Commands}

\begin{itemize}
	\item \emph{env}: MuJoCo Environment ID. Refer Sec. \ref{sec:mujoco_ids}.
	\item \emph{dyn\_params}: Simulation parameters for which the UPN is trained for. Multiple use is possible. Refer Sec. \ref{sec:mujoco_ids}.	
	\item \emph{policy\_path}: path to a trained UPN.
	\item \emph{max\_step}: Maximum step size of training. 		
	\item \emph{seed}: Python random number generators seed.		
	\item \emph{name}: Name of the agent used for saving purposes.
	\item \emph{use\_window}: 1=Use a window based constrained horizon, 0=Use max. default episodic length.
	\item \emph{window\_size}: The window size used as the horizon. Only applicable if $use\_window=1$.
	\item \emph{clip}: clip parameter value of PPO to use.
	\item \emph{lam}: lambda parameter value of PPO to use.
	\item \emph{gamma}: discount factor of learning.
	\item \emph{entcoeff}: an exploration coefficient
	\item \emph{stepsize}: 	learning step-size
	\item \emph{real\_latent}: ground truth simulation parameter values in the real-world (a list saved in a file).	The values used in this project are given in file \emph{reverse\_action\_transform/results/gt\_seed\_0.json}.
	\item \emph{sim\_latent}: ground truth simulation parameter values in the simulator (a list saved in a file).	%\item \emph{batch\_size}: Batch size used for training the UPN
\end{itemize}



\begin{comment}

\subsection{\label{sec:adapt-rat} Adapting \emph{RAT} Policy to the Real-World}

In \emph{policy\_transfer/reality\_mod/rat/rat.py} (at top of the script), change the corresponding lines to following.

\begin{verbatim}
state_noise = (0.3, 0)
DR_noise_resample = False
DR_noise_limits = None
\end{verbatim}

Then run the following scripts for six environments with passing two command line arguments:  1) file path containing the ground-truth parameter values used for \emph{--real\_latent} and \emph{--sim\_latent} and 2) the path to the trained \emph{RAT} initial policy in earlier step which will be used for \emph{--rat\_policy\_path}. Set \emph{Clip}, \emph{Lamda} and \emph{Gamma} parameters to the values listed in Appendix Table 2 for \emph{Adapting RAT}.

\begin{itemize}
\item Ant: \emph{./scripts/train\_rat/ant/ rat\_ant\_5d\_noground.sh}
\item Half-Cheetah: \emph{./scripts/train\_rat/cheetah/ rat\_cheetah\_5d\_noground.sh}
\item Hopper: \emph{./scripts/train\_rat/hopper/ rat\_hopper\_5d\_noground.sh}
\item Humanoid: \emph{./scripts/train\_rat/humanoid/ rat\_humanoid\_5d\_noground.sh}
\item Swimmer: \emph{./scripts/train\_rat/swimmer/ rat\_swimmer\_5d\_noground.sh}
\item Walker2D: \emph{./scripts/train\_rat/walker2d/ rat\_walker\_5d\_noground.sh}
\end{itemize}


\subsection{Common parameters}

\begin{itemize}
	\item \emph{env}: MuJoCo Environment ID. Refer Sec. \ref{sec:mujoco_ids}.
	\item \emph{dyn\_params}: Unknown latent parameters for which the UPN is trained for. Multiple use is possible. Refer Sec. \ref{sec:mujoco_ids}.
	\item \emph{seed}: Python random number generators seed.	
	\item \emph{policy\_path}: Path of the  trained UPN. Refer Sec. \ref{sec:mujoco_ids}.
	\item \emph{samples}: Number of initial policy data points sampled.				
	\item \emph{real\_world}: Trained in real-world (=1) or simulated (=0). Default 0.
	\item \emph{use\_window}: 1=Use a window based constrained horizon, 0=Use max. default episodic length
	\item \emph{window\_size}: The window size used as the horizon. Only applicable if $use\_window=1$.
	
\end{itemize}

\begin{verbatim}
mpirun --map-by socket:OVERSUBSCRIBE 
					-np 6 python policy_transfer/gpbo/run_gpbo.py \
					--env HalfCheetahPT-v2 \
					--batch_size 10000 \ 
					--max_step 200000000  \
					--train_up True  \
					--seed 42 \
					--dyn_params 0 --dyn_params 1 --dyn_params 2 --dyn_params 8 --dyn_params 16 \
					--name mjcheetah5d

\end{verbatim}

\begin{verbatim}
./scripts/train_rat_prior/rat_ant_5d.sh
\end{verbatim}

\subsection{\label{sec:train_transfer} Adapting Transfer Baseline in the Real-world}

To adapt a transfer baseline policy to the real-world (in few shot learning), use the following commands with passing one command line arguments for, 1) the file path containing the ground-truth parameter values used in \emph{--real\_latent}.

\begin{itemize}
\item Ant: \emph{./scripts/update\_upn/uposi\_ant\_5d\_train.sh}
\item Half-Cheetah: \emph{./scripts/update\_upn/uposi\_mjhalfcheetah\_5d\_train.sh}
\item Hopper: \emph{./scripts/update\_upn/uposi\_mjhopper\_5d\_train.sh}
\item Humanoid: \emph{./scripts/update\_upn/uposi\_humanoid\_5d\_train.sh}
\item Swimmer: \emph{./scripts/update\_upn/uposi\_swimmer\_5d\_train.sh}
\item Walker2D: \emph{./scripts/update\_upn/uposi\_mjwalker\_5d\_train.sh}
\end{itemize}
\end{comment}

\begin{comment}
To optimise hyperparameters \emph{clip}, \emph{entcoeff}, \emph{stepsize}, \emph{lambda} and \emph{gamma} for \emph{RAT} adaptation to the real-world, run the following scripts after setting the \emph{RAT} training directives to the following.

\begin{verbatim}
state_noise = (0.3, 0)
DR_noise_resample = False
DR_noise_limits = None
\end{verbatim}

With these commands two command line arguments for, 1) the file path containing the ground-truth parameter values used for \emph{--real\_latent} and \emph{--sim\_latent}, and 2) path to a trained \emph{RAT} initial policy.

\begin{itemize}
\item Ant: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_ant\_5d.sh}
\item Half-Cheetah: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_ant\_5d.sh}
\item Hopper: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_ant\_5d.sh}
\item Humanoid: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_ant\_5d.sh}
\item Swimmer: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_ant\_5d.sh}
\item Walker2D: \emph{./scripts/hyperparams/no\_grounding3/hyperparam\_ant\_5d.sh}
\end{itemize}


\subsection{\label{sec:robust-prior} Trained \emph{Robust RAT Initial Policy}}

In \emph{policy\_transfer/reality\_mod/rat/rat.py} (at top of the script), change the corresponding lines to following. 

\begin{verbatim}
DR_latent_resample = Trie
DR_latent_params = [0, 1] # friction, mass
DR_latent_range = [[0, 0], [1.0, 3.0]] #[low, high]
\end{verbatim}

Then run the following scripts for six environments with passing one command line argument for the file path containing the ground-truth parameter values used for \emph{--real\_latent} and \emph{--sim\_latent}. Please refer to the Section \emph{Parameter Descriptions}. 

%Use the hyperparameter values for \emph{Clip}, \emph{Lamda} and \emph{Gamma} listed in Appendix Table 1 for \emph{Robust RAT initial policy} learning.

\begin{itemize}
\item Ant: \emph{./scripts/train\_rat\_prior/rat\_ant\_5d.sh}
\item Half-Cheetah: \emph{./scripts/train\_rat\_prior/rat\_cheetah\_5d.sh}
\item Hopper: \emph{./scripts/train\_rat\_prior/rat\_hopper\_5d.sh}
\item Humanoid: \emph{./scripts/train\_rat\_prior/rat\_humanoid\_5d.sh}
\item Swimmer: \emph{./scripts/train\_rat\_prior/rat\_swimmer\_5d.sh}
\item Walker2D: \emph{./scripts/train\_rat\_prior/rat\_walker\_5d.sh}
\end{itemize}

\end{comment}


